The CoNFIG Catalogue - II. Comparison of Space Densities in the FR Dichotomy

This paper focuses on a comparison of the space densities of FRI and FRII sources at different epochs, with a particular focus on FRI sources. First, we present the concluding steps in constructing the Combined NVSS-FIRST Galaxy catalogue (CoNFIG), including new VLA observations, optical identifications and redshift estimates. The final catalogue consists of 859 sources over 4 samples (CoNFIG-1, 2, 3 and 4 with flux density limits of S_1.4GHz = 1.3, 0.8, 0.2 and 0.05 Jy respectively). It is 95.7% complete in radio morphology classification and 74.3% of the sources have redshift data. Combining CoNFIG with complementary samples, the distribution and evolution of FRI and FRII sources are investigated. We find that FRI sources undergo mild evolution and that, at the same radio luminosity, FRI and FRII sources show similar space density enhancements in various redshift ranges, possibly implying a common evolution.

==> Contours/jpeg2ps-1.9/Makefile <==
# Makefile for jpeg2ps
# (C) Thomas Merz 1994-2002

VERSION=1.9
DIRNAME = jpeg2ps-$(VERSION)
TARFILE = jpeg2ps-$(VERSION).tar
ZIPFILE = jpeg2ps-$(VERSION).zip

# ----------------------------------------------------------------------------
# Supported compile time options:
# -DA4 gives A4 as default page size, omitting -DA4 gives U.S. letter format
# -DDOS adds DOS and OS/2 support

# The following was reported to work for emx/gcc 0.9c fix04 under OS/2:
# make -f Makefile "CFLAGS=-c -DA4 -DDOS -O2" "LDFLAGS=-Zexe -s"

CFLAGS=-c -DA4
LD=cc
LDFLAGS=
OBJ=o
EXE=
RM=rm -f

.c.$(OBJ) :
	$(CC) $(CFLAGS) $*.c

all:	jpeg2ps$(EXE)

# If your system doesn't have getopt(), add getopt.$(OBJ)
# at the end of the next two lines below.

jpeg2ps$(EXE):	jpeg2ps.$(OBJ) readjpeg.$(OBJ) asc85ec.$(OBJ)
	$(LD) $(LDFLAGS) -o jpeg2ps$(EXE) jpeg2ps.$(OBJ) readjpeg.$(OBJ) asc85ec.$(OBJ)

DISTFILES = \
	jpeg2ps.c psimage.h readjpeg.c asc85ec.c getopt.c	\
	mac_prefix.h						\
	Makefile jpeg2ps.dsp jpeg2ps.mcp			\
	jpeg2ps.txt descrip.mms nesrin.jpg jpeg2ps.1

DOSDISTFILES = $(DISTFILES) jpeg2ps.exe

# Location where to install the binary. This is a suitable value for Linux
# (and possibly other unix-like) systems.
BINDIR = /usr/local/bin

# Location where to install the manual page.
MANDIR = /usr/local/man/man1

CONVFILES = \
	jpeg2ps.c psimage.h readjpeg.c asc85ec.c getopt.c	\
	mac_prefix.h						\
	Makefile jpeg2ps.txt

dist:
	$(RM) $(ZIPFILE) $(TARFILE).gz;				\
	ln -s . $(DIRNAME);					\
	lineend -d $(CONVFILES);		 		\
	(for i in $(DOSDISTFILES); do				\
		echo $$i;					\
	done) | sed "s;.*;$(DIRNAME)/&;" >distfiles;		\
	zip -9 $(ZIPFILE) `cat distfiles`;			\
	(for i in $(DISTFILES); do				\
		echo $$i;					\
	done) | sed "s;.*;$(DIRNAME)/&;" >distfiles;		\
	lineend -u $(CONVFILES); 				\
	tar cvf  $(TARFILE) `cat distfiles`;			\
	gzip -9 $(TARFILE);					\
	$(RM) $(DIRNAME) distfiles;

test:	jpeg2ps$(EXE)
	./jpeg2ps -o nesrin.eps nesrin.jpg

clean:
	$(RM) *.$(OBJ) jpeg2ps$(EXE) $(TARFILE) $(TARFILE).gz $(ZIPFILE) \
	nesrin.eps

install: jpeg2ps$(EXE)
	cp jpeg2ps$(EXE) $(BINDIR)
	cp jpeg2ps.1 $(MANDIR)

uninstall:
	rm -f $(BINDIR)/jpeg2ps$(EXE)
	rm -f $(MANDIR)/jpeg2ps.1

jpeg2ps.$(OBJ):		jpeg2ps.c psimage.h

readjpeg.$(OBJ):	readjpeg.c psimage.h

asc85ec.$(OBJ):		asc85ec.c psimage.h

getopt.$(OBJ):		getopt.c


==> Contours/jpeg2ps-1.9/jpeg2ps.1 <==
.\" This is the manual page for jpeg2ps
.\"
.TH JPEG2PS 1 "Feb 02, 2002" "" ""

.SH NAME
jpeg2ps \- convert JPEG compressed images to PostScript Level 2 or 3

.SH SYNOPSIS
.B jpeg2ps 
[-a] [-b] [-h] [-o 
.I name
] [-p 
.I size
] [-q] [-r
.I dpi
] file.jpg > file.eps

.SH DESCRIPTION
jpeg2ps reads a JPEG file (\fBnot\fP stdin) and writes a DSC-compliant EPS
file containing the compressed JPEG data in PostScript format to stdout.
The produced EPS files contain the necessary DSC comments including
BoundingBox, so they may be imported in page layout applications. However,
they do not contain preview images, so you will only see a gray box on
screen.

The jpeg2ps program performs some sanity checks with the JPEG data. It
detects several kinds of corrupt input data, but it is not absolutely
foolproof. One special feature is that you can feed Macintosh JPEG files
(PICT-JPEG) to jpeg2ps.  These normally have several hundred bytes of
additional stuff before the JPEG data. This PICT rubbish is simply ignored
by jpeg2ps.

.SH OPTIONS
.TP
\fB-a\fP

Auto rotate feature. If the auto rotate feature is activated, images with
width > height are automatically rotated to landscape mode. The image is
scaled in a way to use at least one full edge of the paper. A 20 pt margin
is subtracted on each side. Page sizes can be chosen with the \fB-p\fP
option. The default page size is \fIletter\fP or \fIa4\fP, depending on the
compilation flags. Don't use this option if you simply want to generate EPS
files for inclusion in your documents.

.TP
\fB-b\fP
Binary mode. By default, jpeg2ps sends the image data in ASCII85 encoded
form which is suitable for any communication channel (serial, parallel or
whatever). If you are sure that your channel is truly 8-bit clean,
you can force 8-bit data with this option. Note that this normally does not
apply to 8-bit serial or even parallel channels since some control
characters are reserved for the communications protocol. You can use binary
data e.g.: with some networked printers, with direct-access PostScript
interpreters, e.g. Ghostscript, or serial and parallel channels using
Binary Control Protocol (BCP).

.TP
\fB-h\fP 
Hex mode (ASCIIHex encoding). Using this option, jpeg2ps generates 7-bit
clean data by using ASCIIHex encoding instead of the more space-efficient
ASCII85 encoding.  This is only useful for specialized applications,
e.g. for debugging, since jpeg2ps requires PostScript Level 2 anyway, and
ASCII85 is supported in any Level 2 interpreter.

.TP
\fB-o\fP \fIname\fP
Output file name (as an alternative to output redirection).

.TP
\fB-p\fP \fIsize\fP
Page size name. Known names are: a0, a1, a2, a3, a4, a5, a6, b5, letter,
legal, ledger, p11x17

.TP
\fB-q\fP
Quiet mode: suppress all informational messages

.TP
\fB-r\fP \fIdpi\fP

Resolution value. Using this option you can force jpeg2ps to use a certain
dpi value.  Since automatic actions are also disabled in this case, you are
responsible for choosing a reasonable resolution value.  For example, you
can print a 300 dpi image half-sized by supplying -r 600. 
The option "-r 0" instructs jpeg2ps to look for a JFIF density/resolution
marker and use that value. Automatic scaling and rotation are disabled.
However, if no resolution information is found in the file, jpeg2ps
applies the default algorithm described above.

.SH DIAGNOSTICS
The jpeg2ps program issues three kinds of messages:
.TP
\fBNotes\fP
Have an informational character.
.TP
\fBWarnings\fP
A potential problem with the file was recognized, processing continues.
.TP
\fBErrors\fP
Either a severe problem within the JPEG file was found or the file explores
JPEG features not compatible with PostScript Level 2.

.P
Note that there are some JPEG producers which do not exactly conform to the
specification and that the JPEG spec itself does not cover every aspect of
the file format. You are on the safe side if you demand JFIF files which are
happily accepted by jpeg2ps. (For further information see the JPEG FAQ
by Tom Lane.)

.SH SHAMELESS PLUG
My book contains a lot of information on PostScript, Fonts, and PDF
(currently only available in German):

.nf
Die PostScript- & PDF-Bibel
Von Thomas Merz und Olaf Druemmer
654 Seiten, ISBN 3-935320-01-9
Kopublikation PDFlib GmbH/dpunkt Verlag
http://www.pdflib.com/bibel
e-mail orders: books@pdflib.com

.SH AUTHOR
.nf
Thomas Merz <tm@pdflib.com>
http://www.pdflib.com
.fe

.SH LICENSE
This software is free. You are granted the right to use and copy it. This
software may not be sold or bundled with any commercial package without
express written permission of the author. 

The author accepts no responsibility for damages resulting from the use of
this software and makes no warranty, either express or implied, including but
not limited to, any implied warranty of merchantability or fitness for a
particular purpose. This software is provided as is, and you assume all risks
when using it. 

.\" End of manual page.

